To BERT or Not to BERT: Comparing Task-specific and Task-agnostic Semi-Supervised Approaches for Sequence Tagging

Leveraging large amounts of unlabeled data using Transformer-like architectures, like BERT, has gained popularity in recent times owing to their effectiveness in learning general representations that can then be further fine-tuned for downstream tasks to much success. However, training these models can be costly both from an economic and environmental standpoint. In this work, we investigate how to effectively use unlabeled data: by exploring the task-specific semi-supervised approach, Cross-View Training (CVT) and comparing it with task-agnostic BERT in multiple settings that include domain and task relevant English data. CVT uses a much lighter model architecture and we show that it achieves similar performance to BERT on a set of sequence tagging tasks, with lesser financial and environmental impact.

==> related_work.tex <==
The usefulness of continued training of large transformer-based models on domain/task-related unlabeled data has been shown in recent works \cite{Gururangan2020DontSP, alex2019adapt, xu-etal-2019-bert}, with a varied use of terminology for the process. \cite{xu-etal-2019-bert} and \cite{alex2019adapt} show gains of further tuning BERT \cite{devlin2019bert} using in-domain unlabeled data and refer to this as Post-training, and LM finetuning, respectively. More recently,  \cite{Gururangan2020DontSP} use the term Domain-Adaptive Pretraining and show benefits over RoBERTa \cite{Liu2019RoBERTaAR}. There have also been efforts to reduce model sizes for BERT, e.g. DistilBERT \cite{Sanh2019DistilBERTAD}, these come at some loss in performance (3\%).
